Rigorous Feature Importance Scores based on Shapley Value and Banzhaf Index

Feature attribution methods based on game theory are ubiquitous in the field of eXplainable Artificial Intelligence (XAI). Recent works proposed rigorous feature attribution using logic-based explanations, specifically targeting high-stakes uses of machine learning (ML) models. Typically, such works exploit weak abductive explanation (WAXp) as the characteristic function to assign importance to features. However, one possible downside is that the contribution of non-WAXp sets is neglected. In fact, non-WAXp sets can also convey important information, because of the relationship between formal explanations (XPs) and adversarial examples (AExs). Accordingly, this paper leverages Shapley value and Banzhaf index to devise two novel feature importance scores. We take into account non-WAXp sets when computing feature contribution, and the novel scores quantify how effective each feature is at excluding AExs. Furthermore, the paper identifies properties and studies the computational complexity of the proposed scores.

==> algs/csc-exa.tex <==
%
\begin{algorithmic}[1]

\Procedure{Compute Anytime \xhsc Scores}{$\fml{E}$, `S'}
\State{$(\msf{Fs}^{0}(1), \dots, \msf{Fs}^{0}(m)) \gets (0, \dots, 0)$}
\State{$n \gets 0$}
%
\State{$\fml{Y}_{n+1} \gets \fml{O}_{\mbb{C}}(\fml{E})$}
\Comment{$\fml{O}_{\mbb{C}}(\fml{E})$ returns $\textbf{null}$ if there is no CXp.}
\While{$\fml{Y}_{n+1} \neq \textbf{null}$ AND $\continue(\ldots)$}
\Comment{Customized predicate $\continue(\ldots)$.}
\State{$\tau_{n+1}(\mbf{z}) \gets \tn{ITE}(\sum\limits_{j\in\fml{Y}_{n+1}} z_j > 0, 1, 0) + b_{n+1} \times\prod\limits_{j\in\fml{Y}_{n+1}}(1 - z_j)$}
\State{$w_{n+1} \gets \fml{O}_{\#}(\fml{E}, \fml{Y}_{n+1})$}
\State{\label{alg:csc-exa:ln01}$(\alpha^{n+1}(1), \dots, \alpha^{n+1}(m)) \gets \xsc(w_{n+1} \tau_{n+1}(\mbf{z}), \text{`S'})$}
%
\ForAll{\label{alg:csc-exa:ln02}$i \in \fml{F}$}
\State{\label{alg:csc-exa:ln03}$\msf{Fs}^{n+1}(i) \gets \frac{1}{n+1} (n \msf{Fs}^{n}(i) + \alpha^{n+1}(i))$}
\Comment{Accumulate \xhsc score for each feature.}
\EndFor
\Print{$(\msf{Fs}^{n+1}(1), \dots, \msf{Fs}^{n+1}(m))$}
\Comment{Print updated \xhsc scores for all features.}
%
\State{$n \gets n+1$}
\Comment{Number of CXp increase.}
\State{$\fml{Y} \gets \fml{O}_{\mbb{C}}(\fml{E})$}
\Comment{Get a new CXp.}
\EndWhile
\EndProcedure

\end{algorithmic}




==> algs/cxp-forest01.tex <==
%
\begin{algorithmic}[1] 

\Procedure{Build CXp-Forest}{$\fml{E}$, $\mbb{C}(\fml{E})$}
\For{$\fml{Y}_{i} \in \mbb{C}(\fml{E})$}
\State{Build a DT for $\tau_{i}(\mbf{z}) := \tn{ITE}((\sum\limits_{j\in\fml{Y}_{i}} z_j > 0), 1, b_i)$}
\State{$w_i \gets \#\aex(\fml{Y}_{i})$}
\EndFor
\State{$\tau_{r}(\mbf{z}) := \frac{1}{n} \times \sum\limits_{i=1}^{n} w_i \tau_{i}(\mbf{z})$.}
\State{Let $\fml{M}_{r}$ be the CXp-Forest associated with $\tau_{r}$}
\State{\Return $\fml{M}_{r}$}
\EndProcedure

\end{algorithmic}




==> dtexmpl.tex <==
%\newcommand{\tif}{\tn{IF~}}
%\newcommand{\telse}{\tn{ELSE~}}
%\newcommand{\tthen}{\tn{~THEN~}}
%\newcommand{\tpred}{\msf{predict~}}
\newcommand{\kwpred}{\textbf{Predict~}}

%\begin{figure}[t]
%  \[
%  \begin{array}{l}
%    \tif{x_1}\tthen\\
%    \tif{x_2}\tthen\\
%    \ldots\\
%    \telse
%    \tif{y_1}\tthen \tpred 1\\
%    \telse \tpred 0\\
%    \telse\\
%    \tif{x_2} \tthen \tpred 1\\
%    \telse \tpred 0\\
%  \end{array}
%  \]
%  \caption{Example DT with exponentially many AXps}
%\end{figure}

\begin{algorithm}[t]
  \begin{algorithmic}[1]
    \If{$x_1$}
      \If{$x_2$}
        \If{$x_3$}
          \If{$x_4$}
            \State{$\ldots$}
          \Else % of x4
            \If{$y_2$}
              \State{$\kwpred 1$}
            \Else
              \State{$\kwpred 0$}  
            \EndIf
          \EndIf
        \Else % of x3
          \If{$x_4$}
            \State{$\kwpred 1$}
          \Else
            \State{$\kwpred 0$}
          \EndIf
        \EndIf
      \Else % of x2
        \If{$y_1$}  % left of x2
          \State{$\kwpred 1$}
        \Else
          \State{$\kwpred 0$}  
        \EndIf
      \EndIf
    \Else % of x2
      \If{$x_2$}  % left of x1
        \State{$\kwpred 1$}
      \Else
        \State{$\kwpred 0$}  
      \EndIf
    \EndIf
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
  \begin{algorithmic}[1]
    \If{$x_{2j-1}$}
      \If{$x_{2j}$}
        \State{$\ldots$}
      \Else % of x2j
        \If{$y_j$}  % left of x2j
          \State{$\kwpred 1$}
        \Else
          \State{$\kwpred 0$}
        \EndIf
      \EndIf
    \Else % of x2j
      \If{$x_{2j}$}  % left of x{2j-1}
        \State{$\kwpred 1$}
      \Else
        \State{$\kwpred 0$}  
      \EndIf
    \EndIf
  \end{algorithmic}
  \caption{The gadget used for generating the DT} \label{alg:gadget}
\end{algorithm}

The DT is composed of $k$ gadgets, with $j=1,\ldots,k$, as shown
in~\cref{alg:gadget}.
%
As a result, $m=2k+k$.
%
We can compute the CXps as follows. Each gadget $j$ contributes two
CXps, namely $\{x_{2i-1},x_{2i}\}$ and $\{y_i,x_{2i}\}$.


==> othersc.tex <==

\section{\xhsc scores and CXp-based Deeghan-Packel FISs} \label{app:oscore}
%
We show that, under product distributions over a CXp-Forest, 
there are connections between unweighted \xhsc scores and CXp-based Deeghan-Packel FISs.
%
\begin{restatable}{proposition}{PropUSWffa}
Unweighted Shapley-like \xhsc scores is equivalent to CXp-based Deeghan-Packel FISs.
\end{restatable}
\begin{proof}
Let $|\mbb{C}(\fml{E})| = n$ and $w_i = 1$ for every CXp-tree.
The unweighted Shapley-like \xhsc scores for each relevant feature $j\in\mathfrak{F}(\fml{E})$ is
\begin{equation}
\ufsn{S}(j)
= \frac{1}{n} \sum_{\fml{Y}_{i}\in\mbb{C}(\fml{E}), j\in\fml{Y}_{i}} \frac{1}{|\fml{Y}_{i}|}.
\end{equation}
%
For the same feature $j\in\fml{F}$, its CXp-based Deeghan-Packel FIS is
%
\begin{equation}
\frac{\sum_{\fml{Y}_{i}\in\mbb{C}(\fml{E}), j\in\fml{Y}_{i}} |\fml{Y}_{i}|^{-1} }{|\mbb{C}(\fml{E})|}
= \frac{1}{n} \sum_{\fml{Y}_{i}\in\mbb{C}(\fml{E}), j\in\fml{Y}_{i}} \frac{1}{|\fml{Y}_{i}|}.
\end{equation}
%
Evidently, two scores are the same.
\end{proof}




==> reg_ex.tex <==

\section{Regressor Example} \label{app:reg_ex}
%
\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
\begin{center}
\begin{equation*}
\rho(x_1, x_2, x_3, x_4, x_5) = 0.5 x_1 + 0.25 x_2 + 0.25 x_3 - 0.1 x_4 - 0.1 x_5
\end{equation*}
\end{center}
\caption{Representation of function $\rho$.}
\label{fig:func02}
\end{subfigure}
%
\begin{subfigure}{0.5\textwidth}
\begin{center}
\renewcommand{\arraystretch}{0.95}
\renewcommand{\tabcolsep}{0.5em}
\scalebox{0.95}{\input{./tabs/runex_xp02}}
\end{center}
\caption{XPs of $\fml{E}=(\rho, ((1,1,1,1,1),0.8))$.}
\label{fig:xp02}
\end{subfigure}
\caption{Regressor running example}
\end{figure}

\begin{example}[regression problem] \label{ex:run02a}
Suppose we have a function $\rho$ defined on $\fml{F}=\{1,2,3,4,5\}$ and $\mbb{K}=[0,1]$
where $\mbb{D}_{i} = [0,1]$.
Additionally, assume a continuous uniform distribution $\fml{D}$
with the probability density function $p(x_i)=1$ for each feature $i$.
The function $\rho$ is depicted in~\cref{fig:func02}.
Suppose we are interested in the data point $(\mbf{v},c) = ((1,1,1,1,1),0.8)$.
For the explanation problem $\fml{E}=(\rho, \fml{D}, ((1,1,1,1,1),0.8))$,
suppose the distinguishable threshold $\delta = 0.3$.
\cref{fig:xp02} lists $\mbb{A}(\fml{E})$ and $\mbb{C}(\fml{E})$.
It can be verified that feature 4 and 5 are irrelevant.
\end{example}


\begin{figure}[t]
\begin{center}
\scalebox{.85}{\input{./texfigs/rf02}}
\end{center}
\label{fig:cxpf02}
\caption{Unweight CXp-Forest for $\fml{E}=(\rho, ((1,1,1,1,1),0.8))$.}
\label{fig:rf02}
\end{figure}

\begin{example}\label{ex:run02b}
For the running example~\cref{ex:run02a}, let us consider building an unweighted CXp-Forest.
Assume $\epsilon=0.05$ and we use $\int_{1-\epsilon}^{1} p(x_i) \,dx_i$ to approximate $\prob(z_i=1)$,
then we have $\prob(z_i=1) = 0.05$.
%
Running~\cref{alg:cxp-forest01}, we will obtain an unweighted CXp-Forest as shown in~\cref{fig:rf02},
where $b_1 = \frac{-1}{19}$ and $b_2 = \frac{-39}{361}$.
\end{example}


\begin{example} \label{ex:run02c}
For unweighted CXp-Forest in~\cref{fig:rf02},
consider computing $\ufsn{S}$, then we have
$\ufsn{S}(1) = \frac{1}{2}$, $\ufsn{S}(2) = \frac{1}{4}$, $\ufsn{S}(3) = \frac{1}{4}$, $\ufsn{S}(4) = 0$, and $\ufsn{S}(5) = 0$.
Since all CXps have a size less than 3, $\ufsn{S} = \ufsn{B}$ for any feature.
\end{example}




==> scf.tex <==

\section{Template Scores for Feature Importance} \label{app:scf}
%
This section presents various feature importance template scores defined by~\cite{lhnm-corr2024b}.
These template scores are derived by considering three key components:
1) the subsets of $\fml{F}$ being considered, 
2) the characteristic function being used, and
3) the power index framework employed.

We define the following sets:
\begin{align}
\mbb{WA}_i(\fml{E})&=\{\fml{S}\subseteq\fml{F}\,|\,\waxp(\fml{S};\fml{E})\land{i\in\fml{S}}\}\nonumber\\
\mbb{WC}_i(\fml{E})&=\{\fml{S}\subseteq\fml{F}\,|\,\wcxp(\fml{S};\fml{E})\land{i\in\fml{S}}\}\nonumber\\
\mbb{A}_i(\fml{E})&=\{\fml{S}\subseteq\fml{F}\,|\,\axp(\fml{S};\fml{E})\land{i\in\fml{S}}\}\nonumber\\
\mbb{C}_i(\fml{E})&=\{\fml{S}\subseteq\fml{F}\,|\,\cxp(\fml{S};\fml{E})\land{i\in\fml{S}}\}\nonumber
\end{align}
%
Similarly, we can define $\mbb{WA}$ and $\mbb{WC}$ as the sets of all weak AXps and weak CXps, respectively.
Moreover, let $\Delta(\fml{S};\fml{E},\cf)=\sum_{i\in\fml{S}}\left(\Delta_i(\fml{S};\fml{E},\cf)\right)$.


\paragraph{Template score using Shapley-Shubik power index.}
%
The template Shapley-Shubik score is defined as follows:
%
\begin{equation} \label{eq:tsss}
\tsvn{S}(i; \fml{E}, \cf) := \sum_{\fml{S}\subseteq(\fml{F}\setminus\{i\})}
\left(\frac{\Delta_i(\fml{S};\fml{E},\cf)}{|\fml{F}|\times\binom{|\fml{F}|-1}{|\fml{S}|-1}}\right)
\end{equation}


\paragraph{Template score using Banzhaf power index.}
%
The template Banzhaf score is defined as follows:
%
\begin{equation} \label{eq:tsb}
\tsvn{B}(i;\fml{E},\cf) := \sum_{\fml{S}\subseteq(\fml{F}\setminus\{i\})}
\left(\frac{\Delta_i(\fml{S};\fml{E},\cf)}{2^{|\fml{F}|-1}}\right)
\end{equation}


\paragraph{Template score using Johnston power index.}
%
The template Johnston score is defined as follows:
%
\begin{equation} \label{eq:tsj}
\tsvn{J}(i;\fml{E},\cf) := \sum_{\substack{\fml{S}\subseteq(\fml{F}\setminus\{i\})\\\Delta(\fml{S};\fml{E},\cf)\not=0}}
\left(\frac{\Delta_i(\fml{S};\fml{E},\cf)}{\Delta(\fml{S};\fml{E},\cf)}\right)
\end{equation}


\paragraph{Template score using Deeghan-Packel power index.}
%
The template Deegan-Packel score (equivalent to WFFA~\cite{ignatiev-corr23a,ignatiev-corr23b}) is defined as follows:
%
\begin{equation} \label{eq:tsdp}
\tsvn{D}(i;\fml{E},\cf) := \sum_{\fml{S}\in\mbb{A}_i(\fml{E})}
\left(\frac{\Delta_i(\fml{S};\fml{E},\cf)}{|\fml{S}|\times|\mbb{A}(\fml{E})|}\right)
\end{equation}


\paragraph{Template score using Holler-Packel power index.}
%
The template Holler-Packel score (equivalent to FFA~\cite{ignatiev-corr23a,ignatiev-corr23b}) is defined as follows:
%
\begin{equation} \label{eq:tshp}
\tsvn{H}(i;\fml{E},\cf) := \sum_{\fml{S}\in\mbb{A}_i(\fml{E})}
\left(\frac{\Delta_i(\fml{S};\fml{E},\cf)}{|\mbb{A}(\fml{E})|}\right)
\end{equation}


\paragraph{Template score using Andjiga power index.}
%
The template Andjiga score is defined as follows:
%
\begin{equation} \label{eq:tsa}
\tsvn{A}(i;\fml{E},\cf) := \sum_{\fml{S}\in\mbb{WA}_i}
\left(\frac{\Delta_i(\fml{S};\fml{E},\cf)}{|\fml{S}|\times|\mbb{WA}(\fml{E})|}\right)
\end{equation}




==> tabs/rbo_sum.tex <==

\begin{tabular}{lccc}
\toprule
Compared Scores & Min & Max & Mean \\
\midrule
($\wfsn{S}$, $\wfsn{B}$) & 0.80 & 1.00 & 0.97 \\
($\wfsn{S}$, WFFA) & 0.64 & 1.00 & 0.86 \\
($\wfsn{S}$, SHAP) & 0.46 & 0.89 & 0.75 \\
\midrule
($\wfsn{B}$, WFFA) & 0.56 & 1.00 & 0.85 \\
($\wfsn{B}$, SHAP) & 0.46 & 0.89 & 0.75 \\
\midrule
(WFFA, SHAP) & 0.46 & 0.93 & 0.76 \\
\bottomrule
\end{tabular}


==> tabs/runex_pro01.tex <==

\begin{tabular}{ccl} \toprule
Variable $x_i$ & Value $v_i$ & Probability $\prob(x_i=v_i)$
\\ \toprule
$x_1$    & 0     & $\prob(x_1=0) = 0.25$         \\
$x_1$    & 1     & $\prob(x_1=1) = 0.25$         \\
$x_1$    & 2     & $\prob(x_1=2) = 0.5$         \\
\midrule
$x_2$    & 0     & $\prob(x_2=0) = 0.5$         \\
$x_2$    & 1     & $\prob(x_2=1) = 0.5$         \\
\midrule
$x_3$    & 0     & $\prob(x_3=0) = 0.25$         \\
$x_3$    & 1     & $\prob(x_3=1) = 0.25$         \\
$x_3$    & 2     & $\prob(x_3=2) = 0.5$         \\
\bottomrule
\end{tabular}



==> tabs/runex_xp02.tex <==

\begin{tabular}{cc} \toprule
$\mbb{A}(\fml{E})$ & $\mbb{C}(\fml{E})$
\\ \toprule
$\{1,2\}$     & $\{1\}$     \\
$\{1,3\}$     & $\{2,3\}$     \\
\bottomrule
\end{tabular}




==> texfigs/rf02.tex <==

\forestset{
  my edge/.style={
    edge path={
      \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(0,-5pt) -| (.child anchor)\forestoption{edge label};
    },
  },
  BDT/.style={
    for tree={
      l=1.5cm, s sep=1.15cm,
      if n children=0{}{circle},
      draw=midblue,
      text=midblue,
      edge={my edge},
      edge=thick,
    },
  },
}
%

\begin{forest}
  BDT
  [{$z_1$}, label={[yshift=-6.85ex]{{\tiny1}}},
    edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
    [\dghlight{\textbf{-1/19}}, label={[yshift=-5.125ex]{{\tiny2}}},
      edge label={node[midway,left,xshift=-0.5pt]
        {{\scriptsize$\in\{0\}$}}}, rectangle]
    [\dghlight{\textbf{1}}, label={[yshift=-5.125ex]{{\tiny3}}},
      edge={very thick,draw=darkred}, edge label={node[midway,right,xshift=-0.575pt] {{\scriptsize$\in\{1\}$}}}, rectangle]
  ]
  %
  \node [below=2cm of current bounding box.center] {$w_1=1$};
\end{forest}

\begin{forest}
  BDT
  [{$z_2$}, label={[yshift=-6.85ex]{{\tiny4}}}
    [{$z_3$}, label={[yshift=-6.85ex]{{\tiny5}}},
      edge label={node[midway,left,xshift=-1.5pt] {{\scriptsize$\in\{0\}$}}}
      [\dghlight{\textbf{-39/361}}, label={[yshift=-5.125ex]{{\tiny7}}},
        edge label={node[midway,left,xshift=-0.5pt]
          {{\scriptsize$\in\{0\}$}}}, rectangle]
      [\dghlight{\textbf{1}}, label={[yshift=-5.125ex]{{\tiny8}}},
        edge={very thick,draw=darkred}, edge label={node[midway,right,xshift=-0.575pt] {{\scriptsize$\in\{1\}$}}}, rectangle]
    ]
    [\dghlight{\textbf{1}}, label={[yshift=-5.125ex]{{\tiny6}}},
      edge={very thick,draw=darkred}, edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}},
      rectangle]
  ]
  %
  \node [below=2cm of current bounding box.center] {$w_1=1$};
\end{forest}


